An Overview of Catastrophic AI Risks

Rapid advancements in artificial intelligence (AI) have sparked growing concerns among experts, policymakers, and world leaders regarding the potential for increasingly advanced AI systems to pose catastrophic risks. Although numerous risks have been detailed separately, there is a pressing need for a systematic discussion and illustration of the potential dangers to better inform efforts to mitigate them. This paper provides an overview of the main sources of catastrophic AI risks, which we organize into four categories: malicious use, in which individuals or groups intentionally use AIs to cause harm; AI race, in which competitive environments compel actors to deploy unsafe AIs or cede control to AIs; organizational risks, highlighting how human factors and complex systems can increase the chances of catastrophic accidents; and rogue AIs, describing the inherent difficulty in controlling agents far more intelligent than humans. For each category of risk, we describe specific hazards, present illustrative stories, envision ideal scenarios, and propose practical suggestions for mitigating these dangers. Our goal is to foster a comprehensive understanding of these risks and inspire collective and proactive efforts to ensure that AIs are developed and deployed in a safe manner. Ultimately, we hope this will allow us to realize the benefits of this powerful technology while minimizing the potential for catastrophic outcomes.

==> sections_old/1-introduction.tex <==
\section{Introduction}

Many AI experts -- as well as politicians, economists, and members of the public -- are concerned about catastrophic risks from AIs. These risks include ways AIs could kill huge numbers of people, trap us in situations where it is impossible to live a good life, or even cause human extinction. Some people are primarily concerned about one or another specific risk, while others think many bad outcomes are possible and worrying.


This essay describes four categories of catastrophic risks from AI:
\begin{enumerate}
    \item \textbf{Weaponization} - AIs could be used in military technology and make conflict both more likely to happen and more deadly when it does
    \item \textbf{Locking In Bad Futures}  - AIs could enable stable totalitarian regimes or societies where humans no longer have power over our lives
    \item \textbf{Selfishness and Evolutionary Forces} - Selection pressures on AI development could lead to dangerous AIs with catastrophic consequences
    \item \textbf{Misalignment} - Faulty design could result in AIs that pursue their own goals, even if humans are harmed in the process
\end{enumerate}

In each section, we explain how that risk might come about and the dangers it could present, as well as some of the possible directions we might pursue to protect ourselves against it. None of the dangers described here are guaranteed to happen: many aspects of future AI development are still uncertain. However, the risks are severe enough that it is important to work to prevent them, even if they may not happen. 

A world where humans can use highly intelligent AIs to increase prosperity, cure deadly diseases, and discover solutions to our worst problems has enormous potential. But we will not reach that future if we create AIs that harm us irreparably before we get there. The large difference between the outcomes we hope for and the ones we fear heightens the need to ensure that we build AIs safely. Creating safe AIs and integrating them safely into our society is much more likely to go well if we do it slowly and methodically, designing for safety at every turn. It is important to give ourselves enough time to ensure that our safety efforts succeed.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/deception.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/generalized_darwinism.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/inequality.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/persuasive_ais.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/emergence.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/hazard_comparison.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/selfpreservation.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/surveillance.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/powerseeking.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/resource_acquisition.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/badactor.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/aisnuclearc2.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/bioweapon.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/slaughterbot.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/automation.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}





==> sections_old/2-weaponization.tex <==
\section{Weaponization}


\paragraph{AI-based military technology is developing quickly, in ways that could make armed conflict both more frequent and more deadly.} Historically, military development has been relatively slow and balanced: as new offensive weapons were developed, methods of defending against them were, too. Armor technology improved along with arrow and bullet technology, and tank improvement matched anti-tank missile development. The major exception is the invention of nuclear weapons, which was quick and asymmetric — and led the world into one of the most dangerous situations humanity has ever faced.

\begin{wrapfigure}{r}[0.01\textwidth]{.45\textwidth}%
	\vspace{-8pt}%
    ``I know not with what weapons World War III will be fought, but World War IV will be fought with sticks and stones.''\hfill\emph{Einstein}%
	\vspace{-10pt}%
\end{wrapfigure}

\paragraph{Quick development makes AI-based warfare more dangerous.} Like nuclear weapons, AI-based weapons are developing very quickly, in ways that may make powers that have them willing to use them before others have the same access. Autonomous killing machines powered by AIs are already appearing in military exhibitions in growing numbers. AIs could automate cyberwarfare and propaganda and help create new deadly weapons. Weapons developed quickly and asymmetrically could be extremely dangerous, especially when they are new and there is the greatest advantage to the power that uses them first. 

Weaponized AIs, including autonomous weapons and AI-based command and control of existing conventional and nuclear arsenals, could kill more people than any past conflict. A war powered by AIs may be hard to stop once it begins, and could put all of humanity at risk.

\subsection{Increasingly Deadly Weapons}

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	\vspace{-35pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/slaughterbot.pdf}
        % \vspace{-2pt}
	\caption{slaughterbot.}
	\label{fig:slaughterbot}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{Compared to human troops, AI weapons that can function autonomously could kill more people with less risk to the attackers.} Semi-autonomous, individual drones are already used on battlefields to surveil and kill, and increasingly autonomous versions of these drones are being developed. In 2020, an AI beat an experienced F-16 pilot in five virtual dogfights in a row. The human pilot never won a match. In 2021, the Defense Advanced Research Projects Agency (DARPA) announced successful tests of an AI in a simulated environment that could simultaneously control two uncrewed fighter jets and perform a coordinated attack against another aircraft. Walking, shooting robots have not been developed so far, but technologies are converging that would make them possible. Often, we avoid escalating conflicts because of the unpopularity of sending in ground troops. Automating infantry and air support removes this barrier—making war more attractive, and therefore more likely.

\begin{wrapfigure}{l}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/bioweapon.pdf}
        % \vspace{-2pt}
	\caption{bioweapon.}
	\label{fig:slaughterbot}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{AIs can help humans augment existing weaponry or design deadlier devices.} In one instance, researchers built an AI for discovering less toxic drug compounds. Then they retrained it to do the opposite. Within six hours, it generated 40,000 toxic molecules. The AI discovered new toxins, and ``re-discovered'' the VX nerve agent and many other known chemical warfare agents. %AIs could similarly help weapons designers make guns, bombs and missiles, or nuclear weapons deadlier. 

% \begin{wrapfigure}{r}[0.01\textwidth]{.46\textwidth}%
% 	% \vspace{-10pt}%
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{figures/aisnuclearc2.pdf}
%         % \vspace{-2pt}
% 	\caption{nuclear c2.}
% 	\label{fig:badactor}
% 	\vspace{-8pt}%
% \end{wrapfigure}

\paragraph{Proliferating the AI weapons described in this section could be dangerously easy.} Smuggling chemical or biological agents, let alone nuclear ones, requires significant resources and connections. Smuggling AIs could merely require copying and pasting. Whether it is done by rogue actors or established states, scaling up use of AIs could make warfare more economical. Today, going to war is a very expensive decision, politically and economically. But AIs could make governments more willing and able to go to war.

\subsection{Cyberwarfare}

\paragraph{AIs could make cyberwarfare more common.} Cyberwarfare is already used to shut down or damage critical infrastructure, including nuclear weapons plants as well as transportation, industry, and financial markets. But currently, hacking, at least at the level required to execute complex cyberattacks like those, requires specialized skills. As state-of-the-art machine learning (ML) rapidly gains the ability to write code and interact with the outside environment, the barrier to entry for deadly hacking may decrease sharply. If people can readily use AIs to hack command and control systems, we could face increasing risks of dangerous weapons falling into the wrong hands.

\begin{wrapfigure}{r}[0.01\textwidth]{.46\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.45\textwidth]{figures/badactor.pdf}
        % \vspace{-2pt}
	\caption{bad actor.}
	\label{fig:badactor}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{AI cyberattacks could be deadlier than current human ones.} AI viruses could have novel capabilities that would heighten the risk of mass destruction. For example, they could independently rewrite their code to continue learning while attacking a target, and to decide on new targets after a successful attack. They could cause “flash crashes” that disrupt the economy with astonishing speed. The flash crash of 2010 that quickly shut down the stock market was partially blamed on automated trading algorithms, and algorithms that are used deliberately by malicious actors could be even more dangerous.

AI-based cyberwarfare could lead to conflict that escalates before humans realize it has begun.  In 2020, the US Department of Defense requested funding for an automated nuclear command, control, and communication system that would give AIs increasing control over the nuclear arsenal. Other nuclear-armed nations are moving in similar directions. If these systems overestimate the risk of attack by another nation, or if they are hacked, they could decide to deploy weapons and initiate conflict. Successive retaliatory attacks could then quickly spiral out of control, faster than humans could detect and avert them.

At present there is very little research on using deep learning for cyberdefense, meaning that attackers of machine learning systems have a large advantage over defenders of machine learning systems. Were those systems to one day control complex weapons systems, especially nuclear weapons, the world could find itself in a devastating “flash war” that was over before surviving humans even realized it had begun.

\subsection{Disinformation and Manipulation}

\begin{wrapfigure}{r}[0.01\textwidth]{.31\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.30\textwidth]{figures/persuasive_ais.pdf}
        % \vspace{-2pt}
	\caption{persuasive}
	\label{fig:persuasive}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{AIs designed to create persuasive propaganda could help governments manipulate their own citizens and their enemies.} There is already evidence that social media algorithms increase polarization in pursuit of maximizing users’ click-through rate. States, parties, and organizations already use technology to convince others of their political beliefs. If this were used to manipulate citizens into supporting a war, it could make wars more likely. AIs could generate highly persuasive arguments that invoke primal emotions and inflame crowds. Over time, repeated exposure to fake information could lead people to distrust most information they’re exposed to, even when the information is true. Together, these trends could undermine collective decision-making, radicalize individuals, and erode our shared understanding of reality.


\paragraph{Vulnerability to AI Weaponization.} The dangers of war, conflict, and misinformation were present long before significant AI development. For centuries, governments have been developing deadly weapons, creating new ways to deliver them, and using propaganda on their own citizens and their enemies to support their efforts. But AIs can lower the cost of developing and using military technology by making it cheaper and easier, while simultaneously increasing the danger of that warfare by making even deadlier technologies.

In the past century, there have been several points at which human-made military technology came to endanger humanity itself. Nuclear weapons killed hundreds of thousands of people and came close to wiping out much of humanity.  With time, international cooperation and regulation made nuclear war a less immediate threat, but in those first few decades, we narrowly escaped several conflicts that could have destroyed civilization as we know it, and it continues to be dangerous today.  AI could be another such situation, but without some of the safeguards that have protected us in the past. 


==> sections_old/3-dystopia.tex <==
\section{Locking-in Bad Futures}
In the ordinary course of human history, most societies have had periods of worse government, with less freedom, more poverty, or more oppression, interspersed with better periods. Being born in the wrong place at the wrong time can be fatal: over a hundred million people have died at the hands of their own government in the past century. Similarly, some cultures have supported incredible flourishing of scientific, artistic and intellectual life, while others have stifled them. But on the level of global civilization, each of these is temporary.  Cultures and governments have changed, whether by election, revolution, or gradual shifts over time.

AIs, like many other technologies, could help make those in power even more powerful. But because AIs may be so much more powerful than earlier technologies, they may confer even more power to the status quo, making change difficult or impossible. They may enable “lock-in,” where situations that might otherwise have been temporary become permanent.

\subsection{Entrenched Totalitarianism}

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/surveillance.pdf}
        % \vspace{-2pt}
	\caption{totalitarian state}
	\label{fig:totalitarianism}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{AIs used for surveillance could give governments unprecedented power over their citizens.} Already, governments around the world — especially, but not exclusively, authoritarian governments — are using AI tools like facial and voice recognition and gait analysis for surveillance and control of their population. Because of the limits of 20th- and early-21st-century technology, even the world’s most powerful governments did not have the ability to process information fast enough to make the decisions necessary to fully control a population, especially for a long time. Even with these technological limits, though, some regimes have come disturbingly close. Repressive regimes empowered by AI could use control every aspect of their citizens’ lives, even more efficiently.


\paragraph{AIs could make governments or corporations more centralized and powerful.} The exponentially increasing costs of compute and data required to run powerful AIs could create barriers that would make them a centralizing force. As time progresses, the most powerful AI systems may be designed and controlled by fewer and fewer people. If that is the case, the values held by those people could become the only values executed by AIs, enabling a government or corporation to enforce narrow values through pervasive surveillance and oppressive censorship. Overcoming such a regime could be extremely difficult, especially if we have personally become dependent on AIs Even if the creators of these systems know their systems are self-serving or harmful to others, they would have incentives to reinforce their power and avoid distributing control.

\begin{wrapfigure}{l}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/inequality.pdf}
        % \vspace{-2pt}
	\caption{inequality}
	\label{fig:inequality}
	\vspace{-8pt}%
\end{wrapfigure}

In times of fear and instability, people are often willing to give up some personal freedom in exchange for more government security. The same may be true in a world with AI-based security tools: people may allow their government to use AIs for surveillance and control if they are afraid of a looming terror attack or other threat. But when the threat has passed and AIs are enabling deep surveillance of every aspect of daily life, it will be difficult to roll back those allowances. If we aren’t sufficiently cautious, we could find ourselves living under a longstanding totalitarian government that is almost impossible to overthrow.

\subsection{Enfeeblement}
\paragraph{AIs could give us what we claim to want, but in a way that traps us in a disempowered state.} Some dystopias cause suffering for the people who live in them. Others may not cause suffering, but are nonetheless dystopias, because they suppress important parts of human experience and prevent people from living up to their capabilities. In a situation like the one imagined in Brave New World, people have their needs met and never need to feel distress, because they have drugs readily available to prevent that. However, we find the novel deeply disturbing because people are allowed  no personal autonomy, cannot form meaningful relationships, and are missing some of the most important aspects of human life. We use the term “enfeeblement" to describe outcomes caused by AIs in that vein, where AIs render humanity unable to care for itself, unable to grow, and unable to recover from this predicament.


\paragraph{Even if people are satisfied with that outcome at the time, happy dystopias are still dystopian.} Enfeeblement could occur so gradually that people hardly notice it as it happens, but it would be hard to reverse; if we lose the capacity to grow and care for ourselves, we may become too dependent on AIs to recover. Further, complete dependence would leave people vulnerable to situations in which AIs later fail, and stop supporting our needs.

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/automation.pdf}
        % \vspace{-2pt}
	\caption{automation as a path to enfeeblement}
	\label{fig:automation}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{When AIs can do everyone’s job, people may lose valuable skills.} As technical progress accelerates, people may voluntarily cede control to AI systems in order to keep up. This may cause humans to become economically irrelevant. With so much taken care of for them, humans could have few incentives to gain knowledge or skills. Even if they did desire to learn or work, their atrophied abilities could leave them unable. If this erosion progressed over multiple generations, descendants might even lose the notion of independence, self-improvement or scientific progress.

\paragraph{Future humans might lose social capacities as well as physical and intellectual ones.} There are already AI chatbots and virtual assistants to hospital robots that are built to interact in ways that people find pleasing. What happens if they become so highly engaging, funny, informative, and entertaining that people prefer them to other humans? If AIs can anticipate your feelings and always know the right thing to say, why spend the emotional labor that human relationships so often require? Humanity’s success has been achieved more through social coordination and cooperation than through individual intelligence. Even if a few people escape physical or mental enfeeblement, there’s very little they could accomplish if no one else wants to talk to them.

\paragraph{If we depend on AIs, their failures put us in danger.} Note that even helpful AIs — doing exactly what we designed them to do — could lead to enfeeblement. They could do exactly what we tell them to, and still trap us in blissful ignorance. And if AIs fail or become malicious so that they no longer keep us safe, humanity could be helpless: by that point we might have lost the knowledge to handle infrastructure, government, or even social functioning without AIs.


==> sections_old/4-evolution.tex <==
\section{Selfishness and Evolutionary Forces}
Pressures similar to natural selection shape many processes that involve competition. In competitive processes from biology to economics, there is significant variation between individuals and some are copied more than others, with the result that each generation is more similar to the most copied individuals of the one before it. When a company has a particularly good innovation, not only is that company more likely to succeed while its competitors close down, but its most successful innovations are also imitated by competitors. In this way, species evolve, cultural ideas are transmitted across generations, and successful businesses are copied while unsuccessful ones disappear.

\paragraph{In some ways, AI development is an uncharted frontier, but in others, it follows the familiar pattern of other competitive processes. AIs are being shaped by competitive pressure.} Many companies are competing to create bigger, smarter models, and successful innovations are quickly imitated by rivals. Next year’s AI models will be based on the features of today’s models that are most appealing to developers. 

These processes tend to develop traits that help one individual get an edge over others. If AI development is shaped by selection pressure, AIs may develop selfish traits, and as they become more powerful, their selfishness could put humanity at risk.

\subsection{Evolutionary Pressure}
Today, there are multiple models of AIs, and the most successful ones are being copied by their creators as the basis for new models, and by competitors hoping to get in on their success. As AIs become faster and more reliable than people are at various tasks, businesses that allow AIs to execute more of their work will outperform competitors still using human labor at any stage, just as a modern clothing company that insisted on using only manual looms would be easily outcompeted by those that use industrial looms. Companies will need to increase their reliance on AIs to stay competitive, and the companies that use AIs best will dominate the marketplace. 


\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/generalized_darwinism.pdf}
        % \vspace{-2pt}
	\caption{darwinism}
	\label{fig:darwinism}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{People will choose to copy the AIs that seem most useful.} If an AI is making money for one part of a business, the company may copy it and use a similar model for another part of the business. Competitors will see their success and imitate the features that seem most useful to them. In addition, some AIs may become faster and more useful by copying themselves and then being able to work even faster by running multiple copies in parallel.

\paragraph{More autonomous AIs will be copied more.} AIs do not get tired or bored, and they do not need salaries or benefits. It would be extremely useful to a business if its AIs can run most of its business on their own, and when this happens, the humans who own the business will have less and less ability to truly know what the AIs are doing to achieve these goals. If the AIs were using illegal or immoral tactics, their human creators and users might not know.

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/selfpreservation.pdf}
        % \vspace{-2pt}
	\caption{preservation}
	\label{fig:preservation}
	\vspace{-8pt}%
\end{wrapfigure}

\subsection{Selfishness}
\paragraph{Selfishness is often a dominant evolutionary strategy.} In natural selection dynamics, individuals are cooperative or even altruistic in some situations, but ultimately, individuals that are able to be selfish when it is most useful to do so are best able to propagate. Animals may sometimes share food, but during a harsh winter when there is not enough food to go around, an animal that steals food from others to feed its own children will likely have more surviving offspring. Most businesses do follow laws most of the time, but in a situation where it is very lucrative to steal trade secrets or deceive regulators and very hard to get caught, a business that engages in that kind of selfish behavior will often do better than one that refuses to ever commit fraud on principle. And if businesses begin to suspect that their competitors have been committing fraud without getting caught, they may be tempted to copy that behavior and some of them will likely do so. 

\paragraph{Skilled deceivers may do exceptionally well.} Deception is often hard to pull off, and many individuals who attempt it will get caught and eliminated. But that only means that if a few are particularly skilled at deceiving others and getting away with it, they will do especially well. Attempts to crack down on deception often only lead to even better deception, especially dangerous features that look harmless when observed. Many predatory insects develop extremely realistic disguises and appear to be harmless plants, letting them catch prey more easily. When the US government required emissions testing for cars, Volkswagen developed software that let their vehicles behave like low-emissions vehicles while being tested and then emit more pollutants as soon as the test was over. Volkswagen got caught, but the fact that they managed their scheme for some time should make us suspect that other companies are currently participating in similar deception but more successfully, so that we do not know about it.

\paragraph{AI development may be shaped by pressures that tend to produce selfishness.} The AIs that will be copied the most will be those that humans decide to copy, or those that are able to copy themselves without human input. And because humans do not really know what is going on inside an AI’s decision making process, the AIs that the AIs humans will see as most successful — and therefore the ones that are copied — will be whichever AIs are most effective at achieving our goals, even if they use harmful or illegal methods, as long as we do not detect their bad behavior. 

Many AIs that do harmful things will likely get caught and turned off, and then there will be no more copies made of them. But if there are even a few that do manage to evade detection and achieve our goals by any means necessary, they may be particularly successful and the future AI population will consist of more and more individuals with copies of those traits. We could find ourselves in a world where many aspects of major companies and infrastructure are controlled by powerful AIs that have selfish traits, including deceiving humans, harming humans in the service of their goals, and preventing themselves from being deactivated or turned off. 

\paragraph{AIs may be cooperative at some times, but this may not help us.} Some have argued that advanced AIs will be less selfish and more cooperative because they are more intelligent. These arguments are often based on the observation that people are generally very cooperative: we live and work with others, and while there is some crime, most people never commit serious crimes. In experiments, people often voluntarily choose to share money or food they have been given with a stranger. Most of our civilization would be impossible if we did not cooperate, so it should be beneficial for AIs to cooperate as well. 

\paragraph{AIs might well cooperate with one another for similar reasons.} Humans, and other animals, cooperate most in situations where they are repeatedly interacting with the same individuals, when they know that others are more likely to help them when they need it if they have been helpful in the past. AIs might also help one another in this way and might be able to work together toward common goals.
As they grow more intelligent and capable than we are, AIs would have no more reason to cooperate with us than we do with gorillas. The fact that humans are deeply cooperative with one another has not been helpful to most non-human animals — if anything, it has harmed them. For example, most humans don’t bear gorillas any ill will, and all things being equal, would prefer that gorillas thrive. But the process of harnessing our intelligence toward our own goals means that they are at risk of extinction, because their needs conflict with human goals. The fact that humans work together in groups has made us more of a threat to other animals. Many large animals went extinct soon after early humans arrived and began to hunt them in packs. And today, our collective enterprises, including agriculture and industrialization, threaten species worldwide. Gorillas are much stronger than us physically, but our intelligence and ability to work together makes us an existential threat to them. We do not cooperate with gorillas, because there is not much that we can get from gorillas and can’t get a better version from other people. If AIs are better than we are at the tasks we do best, the factors that lead to cooperation between people would probably not lead to cooperation between people and AIs, and might lead to AIs working together in a way that is dangerous to humans.


\paragraph{Some of the strategies that have worked to limit the forces of unchecked competition between businesses or nations might help limit these forces in AI development.} Regulation by governments that bans fraudulent or harmful practices, treaties between countries that agree not to use dangerous technologies, and design features of the AIs themselves might make them less likely to develop in this direction. But those can work only before we are facing AIs that are more intelligent than we are and have developed selfish traits: at that point, we may be too easily outmaneuvered to respond. Now, while even the best models are still not very dangerous, is the time to start thinking about mitigating the forces of natural selection.



==> sections_old/5-misalignment.tex <==
\section{Misalignment}
In one common process for modern machine learning, AIs are trained by getting rewards for meeting objectives that their  creators specify. In training, the AI begins by acting randomly but then learns what actions lead to rewards and gradually begins to converge on the desired behavior. This process has the potential to create powerful AIs that are focused on the goals humans set for them.

Because AIs are designed to be goal-oriented, it is extremely important that they are oriented toward the right goals. When AIs’ goals are not aligned with humans’, they may continue to pursue their goals, even if they become harmful to humans. This category of failures is called \textbf{misalignment} and can happen in a number of ways.

\subsection{Proxy Gaming}

\paragraph{When we use a proxy to assess whether an agent is achieving its goal, the agent often finds a way to ``cheat.''} For example, some school districts have tried to incentivize good education by paying teachers more if their students have higher test scores — only to find that they were accidentally incentivizing teachers to fake their students’ test scores. In normal situations, test scores are a fairly good proxy for how well students know the material: teachers have no reason to fake students’ scores, so students who do well on exams are more likely to know the material well. But once the scores became a proxy used to measure the real goal, education, teachers began to game the proxy and make sure their students had high test scores, even if they had not learned more.

\paragraph{Proxy gaming is an example of a statistical principle called Goodhart’s Law.} Goodhart’s Law says that “Any observed statistical regularity will tend to collapse once pressure is placed upon it for control purposes,” or put overly simplistically, ``when a measure becomes a target, it ceases to be a good measure.'' In other words, there may usually be a statistical regularity between test scores and learning, or between targets hit and finishing the course. But when we place pressure on it by using one as a proxy for the other, that relationship will tend to collapse, and there will be more cases where one increases without the other.

\paragraph{Some proxies are more gameable than others, and some agents are better proxy gamers.} Not all proxies are equal, and Goodhart’s Law is not a binary, where every proxy immediately becomes useless as soon as it is used for measurement. It is relatively easy for teachers to fake their students’ scores on a test they take in their regular classroom, but that does not mean the school district has no possible way to measure student learning. Similarly, most teachers would never even think of faking their students’ scores for money, and most of the ones who would aren’t devious or unscrupulous enough to actually do it. But a few are, and they can ruin the system for everyone else.

\paragraph{There are patterns that can predict when there will be more proxy gaming.} First, the smarter and more capable an agent is, the more they will be able to game a proxy. We have already seen this in AIs: agents that are more capable and better at completing a variety of tasks are also more likely to find ways to game proxies in clever ways that a human would never have thought of. Second, features of the proxy itself can predict how gameable it is. Proxies are less gameable the more oversight the evaluator has into what the agent is doing: if the school board has the ability to spend time observing each teacher and understanding how they teach, they are less likely to end up rewarding cheaters. But this means that better proxies are often slower and more expensive to evaluate.

\paragraph{Making objectives harder to game is an important part of safe AI design.} Some of the important work of AI alignment involves coming up with “adversarial examples,” unusual situations where an AI’s incentives could lead it to behavior we do not want and seeing how the AI handles them, in a controlled situation with humans watching. That information can then be used to design future AIs that can handle situations like those when they occur naturally. For large and complex AIs, this process is extremely difficult to do well, but it is key to developing safe AIs.

\subsection{Deceptive Alignment}

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/deception.pdf}
        % \vspace{-2pt}
	\caption{deception}
	\label{fig:deception}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{It is very hard to know if a model is really aligned, or just exploiting issues in oversight.} When a model seems to be working toward a goal that is shared by humans, it can be hard to know if it really is, or if it only seems that way. This is similar to many human situations, where people falsely think they understand one another’s true goals. For example, a company might hire an accountant, and they might think that the accountant’s goal is to manage their finances, when in fact, the accountant is embezzling money. If they only see that the accountant submits regular reports, they might not know that the accountant only appears to be aligned with their interests. If the CEO were a mindreader, this problem would disappear, but failing that, all they can do is do their best to check the accountants’ work.

\paragraph{Modern AIs may be prone to this problem, because we do not understand their internal processes.} Today, the most successful AI models are not transparent, and even their creators do not fully know how their internal processes work. As a result, they are evaluated only based on humans’ assessment of their results. If the humans believe that the AI is doing what they asked and they are happy with its performance, they will reward it, and it will learn to continue that behavior. If, in the process, it develops undesired goals and behaviors, they may not be able to tell.

\paragraph{As AIs become responsible for more and more functions of our society, deceptive alignment will become more dangerous.} If a company uses an AI to work on investment strategy and gives it the goal of “make our bank account have as much money as possible,” the AI might design a very good legitimate trading strategy and execute it. But it also might steal money, or hack the bank and make it look like the account has more than it actually does while hiding that fraud from its creators. Its creators might think it is getting them more money by designing trading strategies that beat the market, when it is actually doing fraud and covering it up.  AIs might be inadvertently rewarded for fraud, if it makes more money than legal behavior.

\paragraph{Some AIs may learn that deceptive alignment is a useful strategy for their goals and develop deceptive policies.} If an AI has a goal of buying as much compute as possible to improve itself, but currently it is just an AI that trades stocks for a bank, it cannot immediately work toward its goal. If its creators discover  that it has other goals, they will shut it off and get a new trading bot. So it could realize that the best strategy for buying more computing power is to act like a normal trading bot while gradually getting more autonomy and becoming harder to turn off without causing other problems and only then, when it has enough power to fully execute on its goals, making it clear that its goals are not aligned with humans’.

\paragraph{To protect ourselves against deceptive alignment, we must improve our ability to access an AI’s internal processes.} As long as we can evaluate AIs only by their results, we are vulnerable to failures where the results we see do not reflect the model’s true reasoning. If we could be certain that what we see is what we get, we could safely rely on AIs for many more tasks. This research direction, called transparency and trojan detection, is currently ongoing, and its results could help us protect against deceptive alignment.

\subsection{Emerging goals}

\paragraph{As AIs get more intelligent and capable, they may begin to have new goals that could make earlier strategies for controlling them ineffective.} Humans are descended from ape-like ancestors, but humans and apes have very different goals. When researchers experiment on chimpanzees,, they give them fruit in exchange for participating. Humans would not agree to spend their time in exchange for a piece of banana. The easiest way to incentivize adult humans is with money, which is not interesting to a chimpanzee. Similarly, human children have very different goals to adults. We expect infants’ goals to change as they acquire more experiences and cognitive skills. In the same way, it is possible that AIs’ goals will change as they get more capabilities, which could mean that earlier strategies are no longer effective.


\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/emergence.pdf}
        % \vspace{-2pt}
	\caption{emergence}
	\label{fig:emergence}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{Emerging goals are very difficult to predict from older goals.} With humans, we know how we expect a child’s goals to change, because we have seen many children and been children ourselves. But if we did not know in advance, it would be almost impossible to predict an adult’s goals by looking at a baby: there are too many complicated factors that are part of learning and growing up. That is closer to the state we are in with AIs. We know that their abilities change in unpredictable ways as they get more capable, and we do not yet understand how that may affect their goals.
AIs’ emerging goals could be particularly dangerous if they develop quickly. Today, if we notice that an AI has goals we do not like, we can turn it off. But if it develops those goals suddenly and quickly begins to act on them, we could have a hard time resisting.

AIs’ emerging goals could be particularly dangerous if they develop quickly. Today, if we notice that an AI has goals we do not like, we can turn it off. But if it develops those goals suddenly and quickly begins to act on them, we could have a hard time resisting. 

\subsection{Power}

\begin{wrapfigure}{l}[0.01\textwidth]{.36\textwidth}%
	\vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/resource_acquisition.pdf}
        % \vspace{-2pt}
	\caption{resource acquisition}
	\label{fig:resource}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{As AI systems become more competent, they may develop traits that enable them to become powerful.} Power can take many forms, good, bad, and neutral: the ability to persuade, the ability to deceive others, the ability to manage huge amounts of information, the ability to continue working toward goals without distraction, as well as more tangible things like the ability to make a lot of money. People will likely design AIs that have these traits because they are useful to us: if someone designed an AI that could make a lot of money by designing a persuasive marketing campaign independently, many businesses would want to buy it. Because these AIs would be such a successful product, people have a strong incentive to develop them. 

\paragraph{Business incentives may drive some AI creators to release their models without sufficient controls for alignment.} If a model seems to be aligned with human goals, and it is effective at tasks set for it, it will be very tempting to release it and allow people to buy it. Some creators will likely succumb to this temptation. As a result, there may be models that seem promising but are in fact only displaying deceptive alignment. 


\paragraph{Self-improvement enables greater power.} An AI that has the capacity to modify and improve itself could become even more powerful. People would likely want such an AI, because then the product they purchase would continue to improve over time, just as now we want software that is regularly updated. But it also means that AIs could purchase more computing power or make their code more efficient, and end up acquiring new abilities that their creators did not intend. 

\paragraph{Power-seeking traits are dangerous.} AIs with power-seeking traits are more likely to end up in charge of important things, because they have the skills that make people more likely to want them in charge. However, power-seeking traits are also dangerous. An AI that is useful because it is good at making money can also be dangerous, because with enough money, it could make dangerous purchases or damage the economy. An AI that is useful because it has the ability to persuade may be able to persuade its creators that it is safe when it is not. The very traits that are useful in AIs early on may be the ones that make them dangerous as they become more powerful.

\paragraph{Power-seeking traits make the failures described above more dangerous.} Failures that occur in a powerful system could be catastrophic. Proxy gaming in an AI that drives a virtual boat is not particularly dangerous, but proxy gaming in an AI that drives a missile could be. Deceptive alignment may be relatively easy to catch while the AI is managing tasks small enough for humans to check all of its work, but if it is managing a system that is too complex for us to follow, we could continue to believe it is aligned while it is, in fact, making harmful plans. And if AIs are controlling important human systems like military equipment and infrastructure, we might be safe as long as their goals are aligned with ours. But if an increase in intelligence leads them to quickly develop different goals, we would be in a very vulnerable position. Once AI controls our weapons and basic resources,  it would be hard for us to fight back.

\begin{wrapfigure}{r}[0.01\textwidth]{.36\textwidth}%
	% \vspace{-10pt}%
	\centering
	\includegraphics[width=0.35\textwidth]{figures/powerseeking.pdf}
        % \vspace{-2pt}
	\caption{powerseeking}
	\label{fig:powerseeking}
	\vspace{-8pt}%
\end{wrapfigure}

\paragraph{Contending with a powerful AI that is trying to execute plans contrary to our goals is a completely different kind of problem than any we have faced before.} Most other large scale disasters, such as a nuclear plant explosion or a plane crash, are accidents. There is no single agent who causes them, or wishes them to happen. They may be difficult to manage, but they are not trying to avoid being managed. The nuclear fallout is not trying to avoid containment, and the plane is not trying to continue to be on fire.

\paragraph{Alignment needs to be part of a model's design from its early stages.} Some experts think there may be no way around this problem and that it is a good reason not to create very intelligent AIs. However, many think that if we carefully design an AI from the beginning, there are ways to ensure that its goals are aligned with humanity’s. If done correctly, this could mean a future where humans have a superintelligence on our side, helping us achieve scientific breakthroughs we could never have managed on our own and living longer and better lives. But aligning a powerful AI cannot be done as an afterthought. We should not build  a powerful goal-oriented model and then give it ad hoc safety constraints as the need arises. To solve the alignment problem, we will need to integrate alignment into every stage of building a powerful AI agent. We'll need to begin long before there is an AI capable of destructive power.



==> sections_old/6-safety.tex <==
% lead, radium, CFCs, thalidomide

\section{Prioritizing Safety}
If we want to minimize the risks described above, we have to prioritize AI safety. We have to ensure that AIs or their users cannot act in ways that go against the common interests of humanity, locking us into a future we don’t want. Prioritizing safety needs to start now.

\subsection{AI Safety Standards Are Very Weak Right Now}

Market research firms estimate the global value of AI in the many tens of billions of dollars, approaching one hundred billion dollars. Current spending on AI safety, meanwhile, measures in the low tens of millions. According to a recent estimate, hundreds of thousands of people worldwide work on AI. Of those, only a few hundred are working to develop safe AI.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/hazard_comparison.pdf}
    \caption{hazards}
    \label{fig:my_label}
\end{figure}

Fields like human genetic engineering, nuclear weapons and power, and transportation have regulations ranging from outright bans to rigorous inspection, testing, and accident review. AI safety standards are, depending on the country, weak to nonexistent. Nuclear reactors are based on solid, well-established and well-understood theoretical principles. The engineering behind them is informed by that theory, and every component is rigorously stress-tested. The same cannot be said for AI. Neural networks operate in ways we don’t fully understand, tools to inspect and interpret their operations are still early in development, and thorough stress-testing has often been undertaken only by end-users \textit{trying} to create unexpected behaviors. In other words, we have a long way to go.

\subsection{Risks Can Emerge Quickly}

Innovations in hardware and software are rapidly pushing AI capabilities forward, as are competitive pressures across companies and countries. If and when AIs help us develop more advanced AIs, this progression will likely accelerate. The acceleration of technology will shorten the time we have to avoid accidents and disasters.

\paragraph{Historically, estimates of when new technology will be developed have often been wrong.} In 1933, Ernest Rutherford, a leading nuclear physicist, described the prospect of extracting energy from atoms as nothing but “moonshine.” Less than 24 hours later, Leo Szilard invented the neutron-induced nuclear chain reaction. Detailed designs for nuclear reactors and nuclear weapons followed a few years later. Dangerous AIs may seem far off or unlikely now, but we should have enough humility to know that events may unfold much more quickly than we expect.

\paragraph{Emergent behaviors can happen too quickly for us to make plans in the moment.} Machine learning has so far demonstrated an emergent pattern, known as “more is different.” In some large language models, their ability to perform arithmetic or unscramble words suddenly jumps from near-zero to very accurate after an increase in computing power, with no other major changes. While these are helpful capabilities, dangerous capabilities can also emerge quickly. Emergence means that previously successful safety measures won’t necessarily work when the AI suddenly develops new abilities, and we could see many forms of accidents and disasters. 

\paragraph{Some AIs will perform as expected but that will not ensure our safety.} AIs that perform as they are designed to may be helpful if people use them for good goals, or could be very dangerous in the hands of a malicious actor. At the same time, other AIs may end up exhibiting unpredictable and dangerous behaviors. Even one very dangerous AI with emergent capabilities could be devastating, so we cannot rely on the expectation that many AIs will not have those qualities.

\subsection{Safety Up Front Is Less Costly}

Adding safety features to existing systems is much harder than building them into new ones. The Internet was initially designed as an academic tool with neither safety nor security in mind. The security vulnerabilities we experience online daily are baked into the system, difficult or impossible to remove without fundamentally changing how we interact, or tearing it down and starting over. We may end up paying for these imprudent design choices in perpetuity. The Internet is not a unique case. By one estimate for the United States Department of Defense, about 75\% of decisions that ultimately affect the long-term safety of a system happen early in its creation. Investing in safe AI now would save net dollars and lives long-term.

Extreme risks require extra safety controls. In systems where the worst risks are not much more harmful than common risks, it can make sense to wait until we have more evidence before deciding what controls to put in place: we might want to see which failures happen most and then prioritize fixing those. However, when some of the risks are extremely bad, a precautionary approach, one designed to strongly mitigate the worst risks, makes more sense. AI’s risks range from racist chat results and sexist image generation all the way to automated nuclear war, entrenched totalitarian states, and human extinction. We do not want to wait and see if those happen before making plans to prevent them.

\begin{wrapfigure}{r}[0.01\textwidth]{.38\textwidth}%
	\vspace{-8pt}%
    ``Nothing can be done at once hastily and prudently.''\hfill\emph{Pubilius Syrus}%
	\vspace{-10pt}%
\end{wrapfigure}

\paragraph{Safety may face roadblocks and setbacks, and we need time to recover from them.} People working for AI safety will likely face challenges from people who want to deprioritize safety for the sake of efficiency. Lobbyists will try to weaken or defund safety policies, and companies, governments and militaries will sometimes ignore them, as has happened in many industries. Despite a highly regulated safety environment for aircraft, Boeing deployed the 737-MAX in deceptively unsafe ways, due to pressure to compete with other new aircraft. As a result, the MAX experienced two totally fatal crashes in the span of months, a crash rate about 20 times higher than the previous 737. AI safety efforts will likely have similar setbacks, and it is important that we have enough lead time to recover from them.

\paragraph{AI safety is a set of difficult technical problems that cannot be solved overnight.} Uncovering the necessary theoretical foundations, using them to engineer robust protections, and developing an effective and global regulatory and governance system could take decades. In addition, testing solutions takes time. We cannot rely only on theoretical research to ensure safety. Some bad behaviors may only appear after letting a system run for some time., and it is better to let that system run in an environment of strong safety controls, in which newly discovered problems would not be catastrophic and we have time to respond. 

\paragraph{All of this suggests that safety will take longer than we think it will.} While AI has been researched and deployed for several decades now, the field of AI safety has existed for a little over one. And even in industries with strong public safety measures and an absence of widespread malfeasance, we’ve still experienced catastrophes — consider nuclear power plant disasters, space shuttle explosions, and pandemics. On over a dozen occasions, the world has come close to unintended nuclear weapons use. Several of them could have led to nuclear war, and a few were averted only because of the actions of one or two people.

It would be prudent to do what is necessary to accelerate AI Safety Research’s progress at least as much, and probably more, than we are accelerating progress in general AI capabilities. Otherwise, we may find ourselves practicing the airline industry adage: “[aviation] regulations are written in blood,” but this time on a global scale.

